Integer programming for weakly coupled stochastic dynamic programs with partial information

This paper introduces algorithms for problems where a decision maker has to control a system composed of several components and has access to only partial information on the state of each component. Such problems are difficult because of the partial observations, and because of the curse of dimensionality that appears when the number of components increases. Partially observable Markov decision processes (POMDPs) have been introduced to deal with the first challenge, while weakly coupled stochastic dynamic programs address the second. Drawing from these two branches of the literature, we introduce the notion of weakly coupled POMDPs. The objective is to find a policy maximizing the total expected reward over a finite horizon. Our algorithms rely on two ingredients. The first, which can be used independently, is a mixed integer linear formulation for generic POMDPs that computes an optimal memoryless policy. The formulation is strengthened with valid cuts based on a probabilistic interpretation of the dependence between random variables, and its linear relaxation provide a practically tight upper bound on the value of an optimal history-dependent policies. The second is a collection of mathematical programming formulations and algorithms which provide tractable policies and upper bounds for weakly coupled POMDPs. Lagrangian relaxations, fluid approximations, and almost sure constraints relaxations enable to break the curse of dimensionality. We test our generic POMDPs formulations on benchmark instance forms the literature, and our weakly coupled POMDP algorithms on a maintenance problem. Numerical experiments show the efficiency of our approach.

==> literature.tex <==
%!TEX root=paperRO_arxiv.tex
\section{Literature review}
\label{sec:literature}


%%%%%%%%%%%%%%%%%%Old%%%%%%%%%%%%%%%%%%%
% In the past decades, the optimization in maintenance problems of deteriorating systems have been widely studied in academic research. For a complete description of the various types of maintenance problems, see for instance the surveys of \citet{Flores1989,WANG2002,Alaswad2017}.
% The predictive maintenance problem with capacity constraints belongs to the big family of multistage stochastic optimization problems. Since describing such problems is beyond the scope of this thesis, we refer the interested reader to the tutorial of \citet{powell2014}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Our approach combines a Gaussian HMM with non-interpretable observations, and a fault tree that returns interpretable observations. It leads to a HMM with discrete observations, which are the outputs of a fault tree.
% While HMMs and fault trees give good prediction results independently, our approach combines  
\paragraph{Partially Observable Markov Decision Processes.}
The POMDP framework can be adapted for a wide range of various applications such as maintenance problems \citep{Eckles1968} or clinical decision making \citep{Denton2018}. 
More decision making problems which can be modeled as a POMDP are described in the survey by \citet{Cassandra2003ASO}.
The original POMDP Problem~\ref{pb:POMDP_perfectRecall} has received a lot of interest in the literature, and, the state-of-the-art algorithms solving Problem~\ref{pb:POMDP_perfectRecall} are based on two fundamental results. 
First, a POMDP is equivalent to a MDP in the \emph{belief state} space \cite[Theorem 4]{Eckles1968}. 
The belief state is the posterior probability distribution of the state given past decisions and observations and the belief state space corresponds to the unit simplex. It follows that a POMDP is MDP with a continuous state space and the Bellman's equation can be written on the belief state space (see \cite[Eq. (2.15)]{Krishnamurthy2016}).
The second fundamental result is that the value function of this Bellman's equation is piecewise linear and concave. It enables to derive an exact dynamic programming algorithms for POMDPs with finite \cite{Sondik1973} or infinite horizon \cite{Sondik1978}.
The most important ones are the Witness algorithm \cite{Littman1994,KAELBLING199899} and the Incremental Pruning algorithm \cite{Zhang96,Cassandra97incrementalpruning}. 
However, these exact algorithms become quickly intractable when the size of the spaces grows.
While several heuristics use value function approximations in dynamic programming \cite{Hauskrecht2000,Smith2004}, point-based algorithms approximate the belief state space with a finite subset and derive value iteration on its belief points \cite{Pineau2003,Smith2005,Kurniawati08sarsop,Shani2013}.
\citet{Aras2007} proposed a mixed integer programming approach giving an optimal history-dependent policy that models exactly~\ref{pb:POMDP_perfectRecall}. 
Once again, solving such a program is computationally expensive even for small state spaces and small observation spaces. 
For more details on POMDP solutions, see for instance the surveys of \citet{POMDPMonahan1982,Pineau2008,Shani2013} or more recently the book of \citet{Krishnamurthy2016}.
In a recent work, \citet{Walraven2019} point out the reasons why the existing state-of-the-art algorithms for solving the POMDP problem over infinite horizon with discounted rewards fail to generalize to POMDP problem over a finite horizon without discounting.



%%%%%%%%%%%%%%%%%%%%%%%%OLD%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Modeling a deteriorating system using partially observable continuous time Markov chains has been done in the literature \cite{Makis2003,makis2008,Kim2012,Makis2013}.
% \citet{Kim2011} showed the efficiency of an optimal policy of such a formalization in the mining industry.
% In all these works, the Markov chains have at most three states.
% Many scientific works show that the use of POMDPs to model a maintenance problem gives promising results in practice~\cite{Ellis1995,KIM2018}. In particular, it is showed that modeling the maintenance problem as a POMDP instead of a MDP leads to lower maintenance costs.  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%Old version%%%%%%%%%%%%%
% In our case, we would like to allow a larger number of states to formalize the \maintpb.
% POMDP is known to be PSPACE-complete \cite{Papadimitriou1987}.
% The size of the space grows exponentially with the number of components and experiments using the Julia toolbox show that these POMDP algorithms are not able to solve instances of weakly coupled POMDPs with more than $2$ components. 
% A first step toward a practical solution of the solution was our choice of formalizing the problem.
% We choose to approximate our problem by restricting the set of policies to the set of memoryless policies. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Memoryless policies.} 
% are policies that only depend on the current observation instead of the history of decisions and observations. 
As mentioned in the introduction, in addition to their practical advantages (tractability and easy to apply) the memoryless policies perform well on a broad class of systems in practice \cite{Barto1983,Meuleau1999,Williams1999,Li2011}. 
It has been even proved that for \emph{contextual MDPs}, which are special cases of POMDPs, there always exists an optimal policy that is memoryless \cite{krishnamurthy2016pac}. 
On the other hand, \citet{Littman94memoryless} identifies some pathological cases where the memoryless policies do not work well.
Memoryless policies have received much interest with the increasing popularity of reinforcement learning \cite{Singh1994,Jaakkola1994,Bagnell2004,azizzadeneshelipmlr2016}. Indeed, in this context the decision maker does not have access to the parameters $\pfrak$ and $\bfr.$ Hence, he has to optimize his policy and estimate the parameters at the same time.  
\citet{Azizzadenesheli2016} explain why in this context the memoryless policies are of interest and especially the \emph{stochastic memoryless} policies, which map an observation to a probability distribution over the set of decisions, in opposition to \emph{deterministic memoryless} policies, which map an observation to a decision. 
In particular, the \emph{stationary} policies, i.e., $\delta^t = \delta^1$ for all $t$ in $[T],$ are much more appreciated in the reinforcement learning community \cite{Montufar2015}. 

To solve the POMDP problem with memoryless policy, \citet{Littman94memoryless} proposed a branch-and-bound heuristic that explores the policy space $\Deltaml$ and \citet{Meuleau1999} generalized it into an exact greedy algorithm for solving the problem with infinite horizon and discounted reward. 
In the reinforcement learning community, several policy iteration like algorithms have been proposed to find a stationary stochastic policy \cite{Jaakkola1994,Singh1994,Li2011}. 


\paragraph{Weakly coupled dynamic programs.}
Problem~\ref{pb:decPOMDP_wc} lies in the broad class of multi-stage stochastic optimization problems with high-dimensional state spaces. 
% As mentioned in the introduction, the partially observable multi-armed bandits problems are special case of the weakly coupled POMDP problem.
% When the decision maker observes the states, the problem corresponds to weakly coupled dynamic program. 
Such a problem lies in the broad class of multi-stage stochastic optimization problems that decompose into independent subproblems, which are linked by a collection of coupling constraints on the action space. 
When the decision maker observes the states, each subsystem is a MDP on disjoint state spaces but the actions taken on each subsystem at each time are linked by a coupling constraint.
When these constraints bind weakly, such a problem becomes a weakly coupled dynamic program~\cite{Meuleau1998,Adelman2008}.
It enables to model various types of practical problems such as stochastic inventory routing with limited vehicle capacity \cite{Kleywegt2002}, stochastic multi-product dispatch problems \cite{Papadaki2003}, scheduling problems \cite{Whittle1988}, resources allocation \cite{Gittins1979}, revenue management \cite{Topaloglu2009} and others. More examples can be found for instance in the dissertation of \citet{hawkins2003langrangian}.

It is well known that such a problem can be solved using dynamic programming approach by writing the Bellman's equation. 
Since the size of the state space and action space are exponential in the number of components of the system, the main challenge of solving weakly coupled dynamic programs is the curse of dimensionality as mentioned in Section~\ref{sec:problem}, which makes, in general, the exact dynamic programming approaches intractable. 
% Such a problem is known to be PSPACE-hard \cite{papadimitriou1999}. 
% In particular, in the case of our predictive maintenance problem Problem~\eqref{pb:decPOMDP_wc} corresponds 
To address this challenge, several approximate dynamic programming methods have been proposed \cite{Bertsekas2007,Farias01thelinear,Powell2011,Meuleau1998}. These approaches are mainly based on an approximation of the value functions. Other approaches to solve weakly coupled dynamic program consist in deriving heuristic policies from relaxations. These relaxations are of two types: Lagrangian relaxations of the coupled constraints in the definition ~\eqref{eq:int_prog_weakPOMDP:problem:def_form_action_space} of $\calX_A$ \cite{hawkins2003langrangian,Adelman2008,Ye2018WeaklyCD}, and relaxations of the \emph{non-anticipativity constraints} \cite{Brown2010}, which assume that the decision maker has access to the future outcomes. 
Recently, \citet{bertsimas2016decomposable} gives the tightest upper bound for \emph{decomposable MDPs} with discounted rewards over infinite horizon, which is a more general case where the action space does not necessary decompose along the component action spaces (see remark~\ref{rem:problem:decomposablePOMDP}). 
Their approach and our approach are both based on the linear formulation in terms of moments for Markov Decision Process~\eqref{pb:pomdp:LP_MDP}. 
% The restless multi-armed bandit problem is PSPACE-hard \cite{papadimitriou1999}.

In our case, the decision maker has only access to a partial observation of the arm's state.
If the arms are rested, such a problem has been introduced as POMDP multi-armed bandit problem by \citet{Krishnamurthy09}.
If the arms are restless, like in our maintenance problem, our formalization of the predictive maintenance problem is related to the model considered in the recent works of \citet{Mehta2017}, \citet{MeshramMG18}, \citet{Meshram2019} and \citet{Abbou2019}.
In these works, the model considered has at most two states and three observations.
\citet{Parizi2019} recently proposed a similar framework for weakly coupled POMDP problem where the decision maker maximizes his expected total discounted reward over infinite horizon.

In addition to the curse of dimensionality, the fact that the system is partially observable represents a second challenge.
To address this challenge, new index policies have been proposed \cite{MeshramMG18,KazaMMM2019,Abbou2019}.
Their approach are based on the fact that restless partially observable multi-armed bandit is restless multi-armed bandit where the state space of each component is its belief state space. 
However, the results proposed hold when the state spaces and observation spaces contain at most two elements. Our approach generalizes to bigger state spaces.

% In the case of solving the MDP problem, the classical linear programming formulation~\eqref{pb:LP_MDP} \citep{Epenoux1963} uses the moments of the distribution as variables. This formulation is called "dual formulation" in the book of \citet{Puterman1994} because it is the dual of the well-known linear formulation of the Bellman equation for finite horizon MDP (see e.g. \cite{puterman2014markov}). 

% 
% As mentioned in the introduction,~\ref{pb:decPOMDP_wc} is a weakly coupled dynamic program where the decision maker has only access to partial observations of the system. 

% When the decision maker has access to the system's state,~\ref{pb:decPOMDP_wc} becomes a weakly coupled dynamic program. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%old%%%%%%%%%%%%%%%%%%%%%%%%
% When the decision maker has access to the system's state, the maintenance problem corresponds to the restless multi-armed bandit problem in finite horizon, which is a special case of weakly coupled dynamic program.
% The usual heuristic policies to solve restless multi-armed bandit problem are the \emph{index policies} introduced by \citet{Gittins89}. 
% An index policy consists in computing an index for each arm separately and selecting the arms with the highest indices. It enables to decompose the computation.
% Whittle index policy \cite{Whittle1988} is the most used policy, which is practically efficient in various applications. Other index policies based on polyhedral approaches have been proposed \cite{Bertsimas2000,Bertsimas1996,NinoMora2002}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> literature_v2.tex <==
%!TEX root=paperRO_arxiv.tex
\section{Literature review}
\label{sec:literature}


The problem we consider lies in the broad class of multi-stage stochastic optimization problems with high-dimensional state spaces. 
% When the decision maker observes the arm states, the problem corresponds to a \emph{restless multi-armed bandit}. 
% Such a problem lies in the broad class of multi-stage stochastic optimization problem that decompose into independent subproblems, which are linked by a collection of coupling constraints on the action space. 

When the decision maker observes the states, each subsystem is a MDP on disjoint state spaces but the actions taken on each subsystem at each time are linked by coupled constraints.
When these constraints bind weakly, such a problem is called \emph{weakly coupled dynamic programs} \citep{Meuleau1998,Adelman2008}.
It enables to model various types of practical problems such as stochastic inventory routing with limited vehicle capacity \citep{Kleywegt2002}, stochastic multi-product dispatch problems \citep{Papadaki2003}, scheduling problems \citep{Whittle1988}, resources allocation \citep{Gittins1979}, revenue management \citep{Topaloglu2009} and others. More examples can be found for instance in the dissertation of \citet{hawkins2003langrangian}.
A typical example of weakly coupled dynamic program is the \emph{multi-armed bandit} problem, where a component corresponds to an arm, and at each time step the decision maker has to select a subset of arms to activate in such a way maximizing its expected total reward over finite or infinite horizon.

It is well known that such a problem can be solved using dynamic programming approach by writing the Bellman's equation. 
Since the size of the state space and action space are exponential in the number of components of the system, the main challenge of solving weakly coupled dynamic programs is the curse of dimensionality as mentioned in Section~\ref{sec:problem}, which makes, in general, the exact dynamic programming approaches intractable. 
% Such a problem is known to be PSPACE-hard \cite{papadimitriou1999}. 
% In particular, in the case of our predictive maintenance problem Problem~\eqref{pb:decPOMDP_wc} corresponds 
To address this challenge, several approximate dynamic programming methods have been proposed \cite{Bertsekas2007,Farias01thelinear,Powell2011,Meuleau1998}. These approaches are mainly based on an approximation of the value functions. Other approaches to solve weakly coupled dynamic program consist in deriving heuristic policies from relaxations. These relaxations are of two types: Lagrangian relaxations of the coupling constraints \cite{hawkins2003langrangian,Adelman2008,Ye2014}, and relaxations of the \emph{non-anticipativity constraints} \cite{Brown2010}, which assume that the decision maker has access to the future outcomes. 
Recently, \citet{bertsimas2016decomposable} gives the tightest upper bound for \emph{decomposable MDPs} with discounted rewards over infinite horizon, which is a more general case where the action space does not necessary decompose along the component action spaces. 
Their approach and our approach are both based on the linear formulation in terms of moments for Markov Decision Process~\eqref{pb:pomdp:LP_MDP}. 
% The restless multi-armed bandit problem is a special case of weakly dynamic program partially observed, and is known to be PSPACE-hard \citep{papadimitriou1999}. 
% The usual heuristic policies to solve such a problem are the \emph{index policies}. An index policy consists in computing an index for each arm separately and selecting the arms with the highest indices. Whittle index policy \cite{Whittle1988} is the most used policy, which is practically efficient in various applications.

% \paragraph{Partially Observed Markov Decision Processes.}
% Hence, decision times are already planned and we have new observations (raw data) at each decision time.
In our case, the decision maker has only access to a partial observation of the state, which makes our problem in general at least as difficult as a weakly coupled dynamic program. 

In fact, when there is only one component ($M=1$) the optimization problem becomes a POMDP problem over finite horizon, which is known to be PSPACE-complete \cite{Tsitsiklis1987}. 
State-of-the-art algorithms to solve POMDPs are based on two old results. 
First, a POMDP is equivalent to a continuous state MDP in the \emph{belief state} space \cite[Theorem 4]{Eckles1968}. 
The belief state is the posterior probability distribution of state given past decisions and observations. 
% At each time, the belief state is updated using the belief update formula \citet{Littman1994}[Eq. (1)]. 
Second, leveraging this result, several dynamic programming algorithms have been derived for POMDPs with finite \cite{Sondik1973} or infinite horizon \cite{Sondik1978}. 
More details about these kind of algorithms can be found for instance in the surveys of \citet{POMDPMonahan1982} or more recently the book of \citet{Krishnamurthy2016}.
% wherein the most important ones are the Witness algorithm \cite{Littman1994,KAELBLING199899} and the Incremental Pruning algorithm \cite{Zhang96,Cassandra97incrementalpruning}. However, the exact algorithms become quickly intractable when the size of the spaces grows.
% Hence, approximate algorithms have shown significant improvements.
% While several heuristics use value function approximations in dynamic programming \cite{Hauskrecht2000,Smith2004}, point-based algorithms approximate the belief state space with a finite subset and derive value iteration on its belief points \cite{Pineau2003,Smith2005,Kurniawati08sarsop,Shani2013}.
While the exact algorithms become quickly intractable when the size of the state and observation spaces grow, some approximate algorithms have shown significant improvements. \citet{Hauskrecht2000} and \citet{Pineau2008} survey various approximations methods for POMDPs. 
Many of these (exact or approximate) algorithms for POMDPs have been implemented in an open-source Julia toolbox \cite{Egorov2017}.
In our case, we cannot use these algorithms. Indeed, like MDPs, POMDPs suffer from the \emph{curse of dimensionality}. The size of the space grows exponentially with the number of components and state-of-the art POMDP algorithms are therefore not able to solve instances of our problem with more than $2$ components. 
Hence, we choose to approximate our problem by restricting the set of policies and we use a mathematical programming approach to solve it. \citet{Aras2007} proposed a mixed integer programming approach to exactly solve POMDP problems. 
% In particular, the authors showed that mathematical programming approaches are quite comparable with exact dynamic programming approaches. 
Once again, solving such a program is computationally expensive even for small state spaces and small observation spaces. 
% For more details on POMDP solutions, see for instance the surveys of \citet{POMDPMonahan1982,Pineau2008} or more recently the book of \citet{Krishnamurthy2016}.  
% Many of these algorithms for POMDPs have been implemented in an open-source Julia toolbox \cite{Egorov2017}.
% In our case, these algorithms cannot be applied. Indeed, like MDPs, POMDPs suffer from the \emph{curse of dimensionality}. Hence, the size of the space grows exponentially with the number of components and state-of-the art POMDP algorithms are not able to solve our problem with more than $2$ components. Hence, we choose to approximate our problem by restricting the set of policies.
 % set of \emph{memoryless policies} \cite{Littman94memoryless}, i.e., policies that only depend on the current observation instead of the history of decisions and observations.
% \paragraph{Maintenance of a single component}

% \paragraph{POMDPs in maintenance.}
% The POMDP framework can be adapted for a wide range of various applications\cite{Cassandra2003ASO}, including maintenance problems \cite{Eckles1968}.
% Several structural results on the optimal policy have been proved for deteriorating systems modeled as continuous time Markov chains \cite{Makis2003,makis2008,Kim2012,Makis2013}.
% % Same authors extend this type of result in the case of costly multivariate continuous observations \cite{Kim2012,Makis2013}. 
% In particular, \citet{Makis2003} proved that under technical assumptions the optimal policy is a control limit policy in the belief state space with critical thresholds. 
% \citet{Kim2011} applied this optimal policy in practice.
% However, the model proposed considers only a three states Markov chain. Since our data are highly noisy, a too small number of states leads to a low prediction's accuracy. Our model allows a larger number of degradation states.  

Memoryless policies are policies that only depend on the current observation instead of the history of decisions and observations. 
We choose to solve POMDPs using a memoryless policy for three reasons. 
First, such policy can be easily apply in practice. 
Second, even if finding an optimal memoryless policy remains NP-hard \cite{Littman94memoryless}, the resulting optimization problem is more tractable. 
Third, even if in the general case memoryless policies are not optimal, there is a broad class of systems where memoryless policies perform well \citep{Barto1983,Li2011}. 
\citet{Littman94memoryless} identifies some pathological cases where the memoryless policies do not work well.  
Our problem is in a class of problem where memoryless policies work well because the deterioration process ensures that the input observations will change over time, which does not correspond to the pathological cases of \citet{Littman94memoryless}.
Memoryless policies have received much interest with the increasing popularity of reinforcement learning \citep{Singh1994,Jaakkola1994,Bagnell2004,azizzadeneshelipmlr2016}. 
However, while reinforcement learning algorithms aim at exploring the policy space using \emph{stochastic memoryless policies} \citep{Azizzadenesheli2016}, that map an observation to a probability distribution over the set of decisions, we focus on \emph{deterministic memoryless policies}, that map an observation to a decision. In addition, we allow time-dependent policies instead of the \emph{stationary} policies that are much more appreciated in the reinforcement learning community.   
To the best of our knowledge, there is no compact formulation to find an optimal deterministic memoryless policy for POMDPs.

% \comVC{Peut-être remettre ce paragraphe dans POMDP en deux phrases simples avec les principales références.}
% \paragraph{Weakly coupled dynamic programs.} 
% The optimization problem we consider is also formalized by \citet{MeshramMG18} as a restless partially observed multi-armed bandit. 
% Precisely, a component corresponds to an arm, and at each maintenance slot the decision maker has to select a subset of arms (components) to activate (maintain). 
% The decision maker has only access to a partial observations on each arm. Furthermore, the arms are \emph{restless}, i.e., their state evolves over time even when they are not activated.


When there are more than one component ($M > 1$), in addition to the partially observable aspect of the subsystems, the weakly coupled POMDP problem suffers from the curse of dimensionality as well as the weakly coupled dynamic program.
% the decision maker has only access to a partial observation of the state, which makes our problem in general at least as difficult as a weakly coupled dynamic program. 
\citet{Parizi2019} introduced the weakly coupled POMDP problem where the decision maker maximizes his expected total discounted reward over infinite horizon.
For multi-armed bandit, the optimization problem has been introduced by \citet{MeshramMG18} as \emph{restless partially observed multi-armed bandit} and new index policies have been proposed recently to solve it \citep{MeshramMG18,KazaMMM2019,Abbou2019}. However, the results proposed hold when the state spaces and observation spaces contain at most two elements. Our approach generalizes to any number of states and observations, which gives more flexibility on the learned statistical model while requiring only a moderate computation time.
